Point-Based Value Iteration for POMDPs with Neural Perception Mechanisms

The increasing trend to integrate neural networks and conventional software components in safety-critical settings calls for methodologies for their formal modelling, verification and correct-by-construction policy synthesis. We introduce neuro-symbolic partially observable Markov decision processes (NS-POMDPs), a variant of continuous-state POMDPs with discrete observations and actions, in which the agent perceives a continuous-state environment using a neural {\revise perception mechanism} and makes decisions symbolically. The perception mechanism classifies inputs such as images and sensor values into symbolic percepts, which are used in decision making. We study the problem of optimising discounted cumulative rewards for NS-POMDPs. Working directly with the continuous state space, we exploit the underlying structure of the model and the neural perception mechanism to propose a novel piecewise linear and convex representation (P-PWLC) in terms of polyhedra covering the state space and value vectors, and extend Bellman backups to this representation. We prove the convexity and continuity of value functions and present two value iteration algorithms that ensure finite representability. The first is a classical (exact) value iteration algorithm extending the $\alpha$-functions of Porta {\em et al} (2006) to the P-PWLC representation for continuous-state spaces. The second is a point-based (approximate) method called NS-HSVI, which uses the P-PWLC representation and belief-value induced functions to approximate value functions from below and above for two types of beliefs, particle-based and region-based. Using a prototype implementation, we show the practical applicability of our approach on two case studies that employ (trained) ReLU neural networks as perception functions, by synthesising (approximately) optimal strategies.

==> figures/general_discretisation.tex <==
\begin{figure}[h]
\centering
    \begin{tikzpicture}[scale=0.75]
        \newcommand{\Cross}{$\mathbin{\tikz [x=1.4ex,y=1.4ex,line width=.2ex, red] \draw (0,0) -- (1,1) (0,1) -- (1,0);}$}%
        \newcommand{\Checkmark}{$\color{green}\checkmark$}
        \tikzset{state style/.style={circle, draw, inner sep=0pt,minimum size=20pt}}
        \def\xi{0}
        \def\yi{0}
        %%%
        % first grid scaled down
        % \begin{tikzpicture}[scale=0.75, every node/.style={transform shape}]
        %     \draw[fill = blue!20] (\xi, \yi) rectangle (1,1);
        %     \grid{\xi}{\yi}	
        %     \node [sedan top,body color=red!30,window color=black!80,minimum width=0.75cm, rotate = 90] at (\xi + 0.5, \yi + 0.5) {};
        % \end{tikzpicture}
        %%%
        \draw[fill = blue!20] (\xi, \yi) rectangle (1,1);
            \grid{\xi}{\yi}	
            \node [sedan top,body color=red!30,window color=black!80,minimum width=0.75cm, rotate = 90] at (\xi + 0.5, \yi + 0.5) {};
        \draw[->] (\xi + 0.5, \yi + 0.5) -- (\xi + 0.5, \yi + 1.5) node [pos=1.35, below, xshift=-1.25] {\tiny \textit{up}};
        %
        \def\xi{6}
        \def\yi{0}
        % \filldraw[color=blue] (\xi + 0.5, \yi + 0.75) circle (1.5pt);
        % \filldraw[color=blue] (\xi + 0.5, \yi + 0.25) circle (1.5pt);
        \grid{\xi}{\yi}	
        \draw[black, thin, pattern=north west lines] (\xi + 0.0, \yi + 0.5) rectangle (\xi + 1.0, \yi + 1.5); 
        %
        \def\xi{12}
        \def\yi{0}
        % \filldraw[color=blue] (\xi + 0.5, \yi + 0.75) circle (1.5pt);
        % \filldraw[color=blue] (\xi + 0.5, \yi + 0.25) circle (1.5pt);
        \grid{\xi}{\yi}
        \draw[black, thin, pattern=north west lines] (\xi + 0.0, \yi + 1) rectangle (\xi + 1.0, \yi + 2); 
        %
        \node[state style] (s0) at (0.3,-5.5) {$s_0$};
        \node[state style] (s1) [right=of s0, xshift=-0.9cm] {$s_1$};
        \node[state style] (s2) [right=of s1, xshift=-0.9cm] {$s_2$};
        \node[state style] (s3) [right=of s2, xshift=-0.9cm] {$s_3$};
        \node[state style] (s4) [above=of s0, yshift=-0.9cm] {$s_4$};
        \node[state style] (s5) [right=of s4, xshift=-0.9cm] {$s_5$};
        \node[state style] (s6) [right=of s5, xshift=-0.9cm] {$s_6$};
        \node[state style] (s7) [right=of s6, xshift=-0.9cm] {$s_7$};
        \node[state style] (s8) [above=of s4, yshift=-0.9cm] {$s_8$};
        \node[state style] (s9) [right=of s8, xshift=-0.9cm] {$s_9$};
        \node[state style] (s10) [right=of s9, xshift=-0.9cm] {$s_{10}$};
        \node[state style] (s11) [right=of s10, xshift=-0.9cm] {$s_{11}$};
        \node[state style] (s12) [above=of s8, yshift=-0.9cm] {$s_{12}$};
        \node[state style] (s13) [right=of s12, xshift=-0.9cm] {$s_{13}$};
        \node[state style] (s14) [right=of s13, xshift=-0.9cm] {$s_{14}$};
        \node[state style] (s15) [right=of s14, xshift=-0.9cm] {$s_{15}$};
        \draw[-{Latex[length=1.5mm]}] (s13) + (0.5cm, 1.6cm)  -- node [left] {\scriptsize discrete states} +(0.5cm, 0.7cm);
        %
        \node[state style] (s0-1) at (6.8,-3.7) {$s_0$};
        \node[state style] (s0-2) [above right=of s0-1, xshift=0.2cm, yshift=-0.5cm] {$s_0$};
        \node[state style] (s4-1) [below right=of s0-1, xshift=0.2cm, yshift=+0.5cm] {$s_4$};
        \node[circle, fill, inner sep=1pt] (dN) [right=of s0-1, xshift=-0.5cm] {};
        \draw[-] (s0-1.east) node [above, xshift=0.2cm] {\tiny \textit{up}} -- (dN.center);
        \draw[-{Latex[length=1.5mm]}] (dN.center) -- node [right] {\scriptsize ?} (s0-2.south west);
        \draw[-{Latex[length=1.5mm]}] (dN.center) -- node [right] {\scriptsize ?} (s4-1.north west);
        \draw[-{Latex[length=1.5mm]}] (s0-2) + (-0.8cm, 1.65cm)  -- node [left] {\scriptsize transitions} +(-0.8cm, 0.75cm);
        \node at ([xshift=-1.0cm,yshift=-0.6cm]s4-1) {\Cross};
        %
        \node[state style] (s0-3) at (12.6,-3.7) {$s_0$};
        \node[circle, fill, inner sep=1pt] (dN-1) [right=of s0-3, xshift=-0.5cm] {};
        \node[state style] (s4-2) [right=of s0-3, xshift=0.5cm] {$s_4$};
        \draw[-] (s0-3.east) node [above, xshift=0.2cm] {\tiny \textit{up}} -- (dN-1.center);
        \draw[-{Latex[length=1.5mm]}] (dN-1.center) -- node [above] {\scriptsize 1} (s4-2);
        \draw[-{Latex[length=1.5mm]}] (s0-3) + (1.5cm, 3cm)  -- node [left] {\scriptsize transitions} +(1.5cm, 2cm);
        \node at ([xshift=-3.0em]s4-2.north east)  {};
        \node at ([xshift=-1.7cm,yshift=-2.1cm]s4-2.north east) {\Checkmark};
        %
        \draw[-{Latex[length=1.5mm]}] (4.2, 2)  -- node [above] {\scriptsize image} +(1.2, 0);
        %\draw[-{Latex[length=1.5mm]}] (10.3, 2)  -- node [above] {\scriptsize or image} +(1.2, 0);
        \draw[-{Latex[length=1.5mm]}] (2.0, 4.0) -- (2.0, 4.5) -- node [above,pos=0.5] {\scriptsize or image} (14.0, 4.5) -- (14.0, 4.0);
        % \node[circle, draw] (s0) at (6,-4) {$s_0$};
        % \node[circle, draw] (s1) [above right=of s0, xshift=-0.0cm, yshift=-0.5cm] {$s_1$};
        % \node[circle, draw] (sQ) [below right=of s0, xshift=-0.0cm, yshift=+0.5cm] {$s_?$};
        % \node[circle, fill, inner sep=0.5pt] (dN) [right=of s0, xshift=-0.5cm] {};
        % \draw[-] (s0.east) node [above, xshift=0.2cm] {\tiny \textit{up}} -- (dN.center);
        % \draw[-{Latex[length=1.5mm]}] (dN.center) -- (s1.south west);
        % \draw[-{Latex[length=1.5mm]}] (dN.center) -- (sQ.north west);
        % \draw[black, thin, pattern=north west lines] (\xi + 0.0, \yi + 0.5) rectangle (\xi + 1.0, \yi + 1.5); 
    \end{tikzpicture}
    \caption{{\revise Illustration on why in general, the discretisation cannot work. Left: generate a finite set of discrete states via the perception FCP; middle: if the black image of the blue region under the action $up$ intersects with states that have different percepts, the transition from state $s_0$ under $up$ is ambiguous; right: if the black image intersects with states that have the same percept, then the state $s_0$ is transitioned to $s_4$ with probability $1$ under $up$. There is no prior discretisation of the continuous-state space such that the right case can always hold, which highly depends on the original transition function.}}
    \label{fig:general-discretisation}
\end{figure}

==> figures/parking/4x4_1_initial.tex <==
\begin{figure}[h!]
\centering
\begin{subfigure}{0.49\textwidth}
\includegraphics[width=\textwidth]{figures/parking/4x4_1_initial.png}
\includegraphics[width=\textwidth]{figures/parking/colormap.png}
\end{subfigure}
\begin{subfigure}{0.49\textwidth}
\input{figures/parking/bounds_1.tex}
\end{subfigure}
\caption{Values and strategies.}
\end{figure}

==> figures/parking/4x4_3_initial.tex <==
\begin{figure}[h!]
\centering
\begin{subfigure}{0.49\textwidth}
\includegraphics[width=\textwidth]{figures/parking/4x4_3_initial.png}
\includegraphics[width=\textwidth]{figures/parking/colormap.png}
\end{subfigure}
\begin{subfigure}{0.49\textwidth}
\input{figures/parking/bounds_3.tex}
\end{subfigure}
\caption{Values and strategies.}
\end{figure}

==> figures/parking/4x4_3_initial_obstacle.tex <==
\begin{figure}[h!]
\centering
\begin{subfigure}{0.49\textwidth}
\includegraphics[width=\textwidth]{figures/parking/4x4_3_initial_obstacle.png}
\includegraphics[width=\textwidth]{figures/parking/colormap_obstacle.png}
\end{subfigure}
\begin{subfigure}{0.49\textwidth}
\input{figures/parking/bounds_3_obstacle.tex}
\end{subfigure}
\caption{Values and strategies (obstacle below parking spot).}
\end{figure}

==> figures/parking/advisory-action-table.tex <==
\begin{table*}[t]
% \renewcommand{\arraystretch}{1.5}
\setlength{\tabcolsep}{5pt}  
\centering
\scriptsize{
\begin{tabular}{|c|c||c|c||c|c||c|c|} \hline
Abstract & {\revise Intuitive}  & Abstract & {\revise Intuitive} & Abstract & {\revise Intuitive} &  Abstract & {\revise Intuitive} 
\\
grid {\revise cell} & actions & grid {\revise cell} & actions & grid {\revise cell} & actions & grid {\revise cell} & actions 
\\ \hline \hline	
$(1,1)$ & $\mathit{up}, \mathit{right}$ & $(1,2)$ &   $\mathit{up}, \mathit{right}$ & $(1,3)$ & $\mathit{up}, \mathit{right}$ & $(1,4)$ &  $\mathit{right}$ 
\\
$(2,1)$ & $\mathit{up}, \mathit{right}$ & $(2,2)$ &  $\mathit{up}, \mathit{right}$  & $(2,3)$ & $\mathit{up}, \mathit{right}$ & $(2,4)$ &  $\mathit{right}$ 
\\
$(3,1)$ & $\mathit{up}$  & $(3,2)$ &   $\mathit{up}$ &  $(3,3)$ & $\mathit{up}$ & $(3,4)$ &   $\mathit{park}$ 
\\
$(4,1)$ &  $\mathit{up}, \mathit{left}$ & $(4,2)$ & $\mathit{up}, \mathit{left}$ & $(4,3)$ &  $\mathit{up}, \mathit{left}$ & $(4,4)$ & $\mathit{left}$
\\ \hline
%
\end{tabular}}
\vspace*{-0.0cm}
\caption{{\revise Intuitive} actions of the agent for each percept (abstract grid cell) of the car parking example.}
\label{tab:advisory-parking}
\end{table*}

\iffalse
\begin{table*}[t]
% \renewcommand{\arraystretch}{1.5}
\setlength{\tabcolsep}{5pt}  
\centering
\scriptsize{
\begin{tabular}{|c|l|c|c|} \hline
Cell label & \multirow{2}{*}{Description} & Abstraction grid & \multirow{2}{*}{Suggested actions} \\
$(\per)$ & & (left $\to$ right, bottom $\to$ top) & 
 \\ \hline \hline	
1 & Left bottom to spot & $(1,1)$ & $\mathit{up}, \mathit{right}$
\\
2 & Left bottom to spot & $(2,1)$ & $\mathit{up}, \mathit{right}$ 
\\
3 & Bottom to spot & $(3,1)$ & $up$
\\
4 & Right bottom to spot & $(4,1)$ &  $\mathit{up}, \mathit{left}$
\\
5 & Left bottom to spot & $(1,2)$ &   $\mathit{up}, \mathit{right}$
\\
6 & Left bottom to spot & $(2,2)$ &  $\mathit{up}, \mathit{right}$
\\
7 & Bottom to spot & $(3,2)$ &   $\mathit{up}$
\\
8 & Right bottom to spot & $(4,2)$ & $\mathit{up}, \mathit{left}$
\\ 
9 & Left bottom to spot & $(1,3)$ & $\mathit{up}, \mathit{right}$
\\
10 & Left bottom to spot & $(2,3)$ & $\mathit{up}, \mathit{right}$ 
\\
11 & Bottom to spot &  $(3,3)$ & $\mathit{up}$
\\
12 & Right bottom to spot & $(4,3)$ &  $\mathit{up}, \mathit{left}$
\\
13 & Left to spot & $(1,4)$ &   $\mathit{right}$
\\
14 & Left to spot & $(2,4)$ &  $\mathit{right}$
\\
15 & At spot & $(3,4)$ &   $\mathit{parking}$
\\
16 & Right to spot & $(4,4)$ & $\mathit{left}$
\\ \hline
%
\end{tabular}}
\vspace*{0.2cm}
\caption{Suggested actions for each percept of car parking ($4\times 4$).}
\label{tab:advisory-parking}
\end{table*}
\fi

==> figures/statistics-table.tex <==
\begin{table}[t]
\scriptsize
\setlength{\tabcolsep}{3.5pt}  
\centering
{
\begin{tabular}{|c|c||c|c|c||c|c|} \hline
\multirow{2}{*}{\shortstack[c]{\shortstack[c]{Discount \\ factor}}} & \multirow{2}{*}{\shortstack[c]{\shortstack[c]{Regions \\ $\alpha$-function}}} & \multirow{2}{*}{\shortstack[c]{\shortstack[c]{Comput. \\ time (s)}}}  & \multirow{2}{*}{\shortstack[c]{\shortstack[c]{Lower \\ bound}}} & \multirow{2}{*}{\shortstack[c]{\shortstack[c]{Explore \\ depth}}} &  \multirow{2}{*}{\shortstack[c]{\shortstack[c]{\shortstack[c]{Strategy \\ time (s)}}}} & \multirow{2}{*}{\shortstack[c]{Compatible \\ ratio}} \\ 
 & & & & & & \\ \hline \hline
0.4 & 6278 & 1050.5 & -19.5 & 12 & 495.2 & 18.5\% \\ \hline
0.5 & 5961 & 2477.9 & -227.3 & 14 & 1056.3 & 22.9\% \\ \hline
% 0.52 & 5680 / 6196 & 1204.4 & -294.7 & 16 & 2629.8 & 59.6 \% & 1.85 \\ \hline
0.6 & 6325 & 1079.4 & -481.4 & 21 & 738.7 & 6.8\% \\ \hline
0.7 & 6604 & 2790.8 & -582.2 & 24 &  1377.4 & 33.3 \% \\ \hline
% \hline
%
\end{tabular}}
\vspace*{0.1cm}
\caption{Statistics for the NS-HSVI prototype implementation on the VCAS case study.}
\label{tab:vcas-statistics}
%\vspace*{-0.2cm}
\end{table}
